Versatile Skill Control via Self-supervised Adversarial Imitation of Unlabeled Mixed Motions

Learning diverse skills is one of the main challenges in robotics. To this end, imitation learning approaches have achieved impressive results. These methods require explicitly labeled datasets or assume consistent skill execution to enable learning and active control of individual behaviors, which limits their applicability. In this work, we propose a cooperative adversarial method for obtaining single versatile policies with controllable skill sets from unlabeled datasets containing diverse state transition patterns by maximizing their discriminability. Moreover, we show that by utilizing unsupervised skill discovery in the generative adversarial imitation learning framework, novel and useful skills emerge with successful task fulfillment. Finally, the obtained versatile policies are tested on an agile quadruped robot called Solo 8 and present faithful replications of diverse skills encoded in the demonstrations.

==> plots/mgl/varying_n_z/varying_n_z_cls_10.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle z\)},
xmin=-0.89, xmax=9.89,
xtick style={color=black},
y grid style={darkgray176},
% ylabel={\(\displaystyle \sum_{c}\; p(c \mid \mathbf{o}^{C}_{z})\)},
ymin=0, ymax=1.05000000520065,
ytick style={color=black},
xticks={0,1,2,3,4,5,6,7,8,9},
ymajorticks=false,
]
\draw[draw=none, c0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.002807168379);
\draw[draw=none, c1] (axis cs:-0.4,0.002807168379) rectangle (axis cs:0.4,0.957704431579);
\draw[draw=none, c2] (axis cs:-0.4,0.957704431579) rectangle (axis cs:0.4,0.982601942309);
\draw[draw=none, c3] (axis cs:-0.4,0.982601942309) rectangle (axis cs:0.4,0.990470188092);
\draw[draw=none, c4] (axis cs:-0.4,0.990470188092) rectangle (axis cs:0.4,0.995514411926);
\draw[draw=none, c5] (axis cs:-0.4,0.995514411926) rectangle (axis cs:0.4,0.999999989732);
\draw[draw=none, c0] (axis cs:0.6,0) rectangle (axis cs:1.4,0.0014420711554);
\draw[draw=none, c1] (axis cs:0.6,0.0014420711554) rectangle (axis cs:1.4,0.0050813622934);
\draw[draw=none, c2] (axis cs:0.6,0.0050813622934) rectangle (axis cs:1.4,0.9890064489934);
\draw[draw=none, c3] (axis cs:0.6,0.9890064489934) rectangle (axis cs:1.4,0.9976802182304);
\draw[draw=none, c4] (axis cs:0.6,0.9976802182304) rectangle (axis cs:1.4,0.9995347401191);
\draw[draw=none, c5] (axis cs:0.6,0.9995347401191) rectangle (axis cs:1.4,0.9999999882621);
\draw[draw=none, c0] (axis cs:1.6,0) rectangle (axis cs:2.4,0.0016787479786);
\draw[draw=none, c1] (axis cs:1.6,0.0016787479786) rectangle (axis cs:2.4,0.0066997806306);
\draw[draw=none, c2] (axis cs:1.6,0.0066997806306) rectangle (axis cs:2.4,0.007953219341);
\draw[draw=none, c3] (axis cs:1.6,0.007953219341) rectangle (axis cs:2.4,0.152639774641);
\draw[draw=none, c4] (axis cs:1.6,0.152639774641) rectangle (axis cs:2.4,0.992196690141);
\draw[draw=none, c5] (axis cs:1.6,0.992196690141) rectangle (axis cs:2.4,1.000000004953);
\draw[draw=none, c0] (axis cs:2.6,0) rectangle (axis cs:3.4,0.002537700542);
\draw[draw=none, c1] (axis cs:2.6,0.002537700542) rectangle (axis cs:3.4,0.00447171841);
\draw[draw=none, c2] (axis cs:2.6,0.00447171841) rectangle (axis cs:3.4,0.011316003618);
\draw[draw=none, c3] (axis cs:2.6,0.011316003618) rectangle (axis cs:3.4,0.987175759418);
\draw[draw=none, c4] (axis cs:2.6,0.987175759418) rectangle (axis cs:3.4,0.991562056816);
\draw[draw=none, c5] (axis cs:2.6,0.991562056816) rectangle (axis cs:3.4,0.999999975651);
\draw[draw=none, c0] (axis cs:3.6,0) rectangle (axis cs:4.4,0.0004869177049);
\draw[draw=none, c1] (axis cs:3.6,0.0004869177049) rectangle (axis cs:4.4,0.0020105445639);
\draw[draw=none, c2] (axis cs:3.6,0.0020105445639) rectangle (axis cs:4.4,0.0028920020534);
\draw[draw=none, c3] (axis cs:3.6,0.0028920020534) rectangle (axis cs:4.4,0.0076407177434);
\draw[draw=none, c4] (axis cs:3.6,0.0076407177434) rectangle (axis cs:4.4,0.0097357700374);
\draw[draw=none, c5] (axis cs:3.6,0.0097357700374) rectangle (axis cs:4.4,0.9999999959374);
\draw[draw=none, c0] (axis cs:4.6,0) rectangle (axis cs:5.4,0.7456892235);
\draw[draw=none, c1] (axis cs:4.6,0.7456892235) rectangle (axis cs:5.4,0.81534221391);
\draw[draw=none, c2] (axis cs:4.6,0.81534221391) rectangle (axis cs:5.4,0.98962899621);
\draw[draw=none, c3] (axis cs:4.6,0.98962899621) rectangle (axis cs:5.4,0.99280948937);
\draw[draw=none, c4] (axis cs:4.6,0.99280948937) rectangle (axis cs:5.4,0.998943239678);
\draw[draw=none, c5] (axis cs:4.6,0.998943239678) rectangle (axis cs:5.4,0.9999999864622);
\draw[draw=none, c0] (axis cs:5.6,0) rectangle (axis cs:6.4,0.003372372887);
\draw[draw=none, c1] (axis cs:5.6,0.003372372887) rectangle (axis cs:6.4,0.984027033287);
\draw[draw=none, c2] (axis cs:5.6,0.984027033287) rectangle (axis cs:6.4,0.986639111741);
\draw[draw=none, c3] (axis cs:5.6,0.986639111741) rectangle (axis cs:6.4,0.994295424908);
\draw[draw=none, c4] (axis cs:5.6,0.994295424908) rectangle (axis cs:6.4,0.997715154604);
\draw[draw=none, c5] (axis cs:5.6,0.997715154604) rectangle (axis cs:6.4,0.9999999748);
\draw[draw=none, c0] (axis cs:6.6,0) rectangle (axis cs:7.4,0.001472741837);
\draw[draw=none, c1] (axis cs:6.6,0.001472741837) rectangle (axis cs:7.4,0.004093485056);
\draw[draw=none, c2] (axis cs:6.6,0.004093485056) rectangle (axis cs:7.4,0.006601249333);
\draw[draw=none, c3] (axis cs:6.6,0.006601249333) rectangle (axis cs:7.4,0.0077477990617);
\draw[draw=none, c4] (axis cs:6.6,0.0077477990617) rectangle (axis cs:7.4,0.9992197401617);
\draw[draw=none, c5] (axis cs:6.6,0.9992197401617) rectangle (axis cs:7.4,0.999999981657);
\draw[draw=none, c0] (axis cs:7.6,0) rectangle (axis cs:8.4,0.8681531537);
\draw[draw=none, c1] (axis cs:7.6,0.8681531537) rectangle (axis cs:8.4,0.871195131779);
\draw[draw=none, c2] (axis cs:7.6,0.871195131779) rectangle (axis cs:8.4,0.8723165741257);
\draw[draw=none, c3] (axis cs:7.6,0.8723165741257) rectangle (axis cs:8.4,0.9966486978957);
\draw[draw=none, c4] (axis cs:7.6,0.9966486978957) rectangle (axis cs:8.4,0.9996612749347);
\draw[draw=none, c5] (axis cs:7.6,0.9996612749347) rectangle (axis cs:8.4,0.9999999830635);
\draw[draw=none, c0] (axis cs:8.6,0) rectangle (axis cs:9.4,0.8447248744);
\draw[draw=none, c1] (axis cs:8.6,0.8447248744) rectangle (axis cs:9.4,0.97042180267);
\draw[draw=none, c2] (axis cs:8.6,0.97042180267) rectangle (axis cs:9.4,0.985492841025);
\draw[draw=none, c3] (axis cs:8.6,0.985492841025) rectangle (axis cs:9.4,0.990954290185);
\draw[draw=none, c4] (axis cs:8.6,0.990954290185) rectangle (axis cs:9.4,0.998775027167);
\draw[draw=none, c5] (axis cs:8.6,0.998775027167) rectangle (axis cs:9.4,0.999999979366);
\end{axis}

\end{tikzpicture}


==> plots/sgl/master_cls_over_time_aligned/sgl/ratio/ratio_ratio_10.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={z},
xmin=-0.69, xmax=5.69,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(wave \mid z)\)},
ymin=0, ymax=0.01067733740955,
ytick style={color=black}
]
\draw[draw=none, z0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.005257126888);
\draw[draw=none, z1] (axis cs:0.6,0) rectangle (axis cs:1.4,0.010168892771);
\draw[draw=none, z2] (axis cs:1.6,0) rectangle (axis cs:2.4,0.0017355491946);
\draw[draw=none, z3] (axis cs:2.6,0) rectangle (axis cs:3.4,0.005196912958);
\draw[draw=none, z4] (axis cs:3.6,0) rectangle (axis cs:4.4,0.0018763206481);
\draw[draw=none, z5] (axis cs:4.6,0) rectangle (axis cs:5.4,0.009953058427);
\end{axis}

\end{tikzpicture}


==> plots/sgl/master_cls_over_time_aligned/sgl/ratio/ratio_ratio_1000.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={z},
xmin=-0.69, xmax=5.69,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(wave \mid z)\)},
ymin=0, ymax=1.041863729865,
ytick style={color=black}
]
\draw[draw=none, z0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.0016888943885);
\draw[draw=none, z1] (axis cs:0.6,0) rectangle (axis cs:1.4,0.0020539207437);
\draw[draw=none, z2] (axis cs:1.6,0) rectangle (axis cs:2.4,0.005399503501);
\draw[draw=none, z3] (axis cs:2.6,0) rectangle (axis cs:3.4,0.003317005703);
\draw[draw=none, z4] (axis cs:3.6,0) rectangle (axis cs:4.4,0.9922511713);
\draw[draw=none, z5] (axis cs:4.6,0) rectangle (axis cs:5.4,0.0022821089041);
\end{axis}

\end{tikzpicture}


==> plots/sgl/master_cls_over_time_aligned/sgl/ratio/ratio_ratio_200.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={z},
xmin=-0.69, xmax=5.69,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(wave \mid z)\)},
ymin=0, ymax=0.022962110619,
ytick style={color=black}
]
\draw[draw=none, z0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.0019472099116);
\draw[draw=none, z1] (axis cs:0.6,0) rectangle (axis cs:1.4,0.011869480853);
\draw[draw=none, z2] (axis cs:1.6,0) rectangle (axis cs:2.4,0.0015996117712);
\draw[draw=none, z3] (axis cs:2.6,0) rectangle (axis cs:3.4,0.007799447967);
\draw[draw=none, z4] (axis cs:3.6,0) rectangle (axis cs:4.4,0.014079854171);
\draw[draw=none, z5] (axis cs:4.6,0) rectangle (axis cs:5.4,0.02186867678);
\end{axis}

\end{tikzpicture}


==> plots/sgl/master_cls_over_time_aligned/sgl/skill_switch/skill_switch.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle t\)},
xmin=-26.25, xmax=551.25,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(c \mid \mathbf{o}^{C}_{z})\)},
ymin=-0.0599999999944802, ymax=1.25999999999974,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {opts_str}{skill_switch-000.dat};
\addplot [semithick, darkorange25512714]
table {opts_str}{skill_switch-001.dat};
\addplot [semithick, forestgreen4416044]
table {opts_str}{skill_switch-002.dat};
\addplot [semithick, crimson2143940]
table {opts_str}{skill_switch-003.dat};
\addplot [semithick, mediumpurple148103189]
table {opts_str}{skill_switch-004.dat};
\addplot [semithick, sienna1408675]
table {opts_str}{skill_switch-005.dat};
\path [draw=steelblue31119180, line width=2pt]
(axis cs:0,1.2)
--(axis cs:75,1.2);

\path [draw=steelblue31119180, line width=2pt]
(axis cs:75,1.2)
--(axis cs:150,1.2);

\path [draw=steelblue31119180, line width=2pt]
(axis cs:150,1.2)
--(axis cs:225,1.2);

\path [draw=steelblue31119180, line width=2pt]
(axis cs:225,1.2)
--(axis cs:300,1.2);

\path [draw=steelblue31119180, line width=2pt]
(axis cs:300,1.2)
--(axis cs:375,1.2);

\path [draw=steelblue31119180, line width=2pt]
(axis cs:375,1.2)
--(axis cs:450,1.2);

\path [draw=steelblue31119180, line width=2pt]
(axis cs:450,1.2)
--(axis cs:525,1.2);

\end{axis}

\end{tikzpicture}


==> plots/sgl/ratio/ratio.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\# of trajectories},
xmin=-48.95, xmax=1049.95,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle \max\{p(\mathrm{wave} \mid \mathbf{o}^{C}_{z})\}\)},
ymin=-0.242094316122182, ymax=1.25780684777772,
ytick style={color=black}
]
\path [fill=black, fill opacity=0.5]
(axis cs:1,0.0150679705308088)
--(axis cs:1,0.0108750668299912)
--(axis cs:10,0.0112507409885374)
--(axis cs:20,0.0104185003206975)
--(axis cs:50,0.0112802095626647)
--(axis cs:100,0.0134149359154233)
--(axis cs:200,-0.173916990490368)
--(axis cs:250,0.00980552193572808)
--(axis cs:300,0.973244771764334)
--(axis cs:350,0.988468836263417)
--(axis cs:400,0.990180116051193)
--(axis cs:450,0.990458709030853)
--(axis cs:500,0.989891455338674)
--(axis cs:800,0.396541743134089)
--(axis cs:1000,0.991580282105707)
--(axis cs:1000,0.992453813494292)
--(axis cs:1000,0.992453813494292)
--(axis cs:800,1.18962952214591)
--(axis cs:500,0.992301469341326)
--(axis cs:450,0.991208433569147)
--(axis cs:400,0.991388231868807)
--(axis cs:350,0.990642994936583)
--(axis cs:300,0.992042914355666)
--(axis cs:250,0.0407386048870719)
--(axis cs:200,0.588594913721168)
--(axis cs:100,0.0218172015469767)
--(axis cs:50,0.0147305684453353)
--(axis cs:20,0.0202345832269025)
--(axis cs:10,0.0146424361706626)
--(axis cs:1,0.0150679705308088)
--cycle;

\addplot [black]
table {plots/sgl/ratio/ratio-000.dat};
\end{axis}

\end{tikzpicture}

==> plots/sgl/ratio/ratio_ratio_10.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$z$},
xmin=-0.69, xmax=5.69,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(\text{wave} \mid \mathbf{o}^{C}_{z})\)},
ymin=0, ymax=0.01067733740955,
ytick={0.002, 0.006, 0.01},
ytick style={color=black}
]
\draw[draw=none, z0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.005257126888);
\draw[draw=none, z1] (axis cs:0.6,0) rectangle (axis cs:1.4,0.010168892771);
\draw[draw=none, z2] (axis cs:1.6,0) rectangle (axis cs:2.4,0.0017355491946);
\draw[draw=none, z3] (axis cs:2.6,0) rectangle (axis cs:3.4,0.005196912958);
\draw[draw=none, z4] (axis cs:3.6,0) rectangle (axis cs:4.4,0.0018763206481);
\draw[draw=none, z5] (axis cs:4.6,0) rectangle (axis cs:5.4,0.009953058427);
\end{axis}

\end{tikzpicture}


==> plots/sgl/ratio/ratio_ratio_1000.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$z$},
xmin=-0.69, xmax=5.69,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(\text{wave} \mid \mathbf{o}^{C}_{z})\)},
ymin=0, ymax=1.0,
ytick={0.2,0.6,1.0},
ytick style={color=black}
]
\draw[draw=none, z0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.0016888943885);
\draw[draw=none, z1] (axis cs:0.6,0) rectangle (axis cs:1.4,0.0020539207437);
\draw[draw=none, z2] (axis cs:1.6,0) rectangle (axis cs:2.4,0.005399503501);
\draw[draw=none, z3] (axis cs:2.6,0) rectangle (axis cs:3.4,0.003317005703);
\draw[draw=none, z4] (axis cs:3.6,0) rectangle (axis cs:4.4,0.9922511713);
\draw[draw=none, z5] (axis cs:4.6,0) rectangle (axis cs:5.4,0.0022821089041);
\end{axis}

\end{tikzpicture}


==> plots/sgl/ratio/ratio_ratio_200.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}


\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={z},
xmin=-0.69, xmax=5.69,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle p(wave \mid z)\)},
ymin=0, ymax=0.022962110619,
ytick style={color=black}
]
\draw[draw=none, z0] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.0019472099116);
\draw[draw=none, z1] (axis cs:0.6,0) rectangle (axis cs:1.4,0.011869480853);
\draw[draw=none, z2] (axis cs:1.6,0) rectangle (axis cs:2.4,0.0015996117712);
\draw[draw=none, z3] (axis cs:2.6,0) rectangle (axis cs:3.4,0.007799447967);
\draw[draw=none, z4] (axis cs:3.6,0) rectangle (axis cs:4.4,0.014079854171);
\draw[draw=none, z5] (axis cs:4.6,0) rectangle (axis cs:5.4,0.02186867678);
\end{axis}

\end{tikzpicture}

